Fork is All You Need in Heterogeneous Systems

We present a unified programming model for heterogeneous computing systems. Such systems integrate multiple computing accelerators and memory units to deliver higher performance than CPU-centric systems. Although heterogeneous systems have been adopted by modern workloads such as machine learning, programming remains a critical limiting factor. Conventional heterogeneous programming techniques either impose heavy modifications to the code base or require rewriting the program in a different language. Such programming complexity stems from the lack of a unified abstraction layer for computing and data exchange, which forces each programming model to define its abstractions. However, with the emerging cache-coherent interconnections such as Compute Express Link, we see an opportunity to standardize such architecture heterogeneity and provide a unified programming model. We present CodeFlow, a language runtime system for heterogeneous computing. CodeFlow abstracts architecture computation in programming language runtime and utilizes CXL as a unified data exchange protocol. Workloads written in high-level languages such as C++ and Rust can be compiled to CodeFlow, which schedules different parts of the workload to suitable accelerators without requiring the developer to implement code or call APIs for specific accelerators. CodeFlow reduces programmers' effort in utilizing heterogeneous systems and improves workload performance.

==> Makefile <==
projects := $(PWD)
all_targets += paper.pdf
root_path := $(PWD)
include common.mk

# include project/conference/usenix.mk

# project/conference/usenix.mk: project/conference/usenix.csv
# 	cd project/conference && python3 configure.py

.PHONY: testoutput
testoutput:
	echo $(projects)

.DEFAULT_GOAL:=all_projects

.PHONY: all_projects
all_projects: build_all_projects

.PHONY: build_all_projects
build_all_projects: paper.pdf
	# @for dir in $(projects); do \
	# 	$(MAKE) -s --no-print-directory -C $$dir all; \
	# done
	@echo "ALL FINISHED"

.PHONY: clean_projects
clean_projects:
	for dir in $(projects); do \
		$(MAKE) -C $$dir clean; \
	done

.PHONY: distclean_projects
distclean_projects:
	for dir in $(projects); do \
		$(MAKE) -C $$dir distclean; \
	done

arxiv.zip: build_all_projects
	git archive --format=zip HEAD >$@
	zip -ur $@ paper.bbl


==> config/style/colors.tex <==
\@ifpackageloaded{xcolor}
    {}
    {\usepackage[dvipsnames]{xcolor}}

% Sunset from Carto Color
% #f3e79b,#fac484,#f8a07e,#eb7f86,#ce6693,#a059a0,#5c53a5
\definecolor{SunsetI}   {HTML}{f3e79b}
\definecolor{SunsetII}  {HTML}{fac484}
\definecolor{SunsetIII} {HTML}{f8a07e}
\definecolor{SunsetIV}  {HTML}{eb7f86}
\definecolor{SunsetV}   {HTML}{ce6693}
\definecolor{SunsetVI}  {HTML}{a059a0}
\definecolor{SunsetVII} {HTML}{5c53a5}

% SunsetDark from Carto Color
% #fcde9c,#faa476,#f0746e,#e34f6f,#dc3977,#b9257a,#7c1d6f
\definecolor{SunsetDarkI}   {HTML}{fcde9c}
\definecolor{SunsetDarkII}  {HTML}{faa476}
\definecolor{SunsetDarkIII} {HTML}{f0746e}
\definecolor{SunsetDarkIV}  {HTML}{e34f6f}
\definecolor{SunsetDarkV}   {HTML}{dc3977}
\definecolor{SunsetDarkVI}  {HTML}{b9257a}
\definecolor{SunsetDarkVII} {HTML}{7c1d6f}


==> config/style/draft.tex <==

% % Don't use `todonote` package, it slows down the LaTeX compilation
% % Treat todo as text or not
% \ifthenelse{\boolean{todoastext}}{
%     % Output todo as text
%     \newcommand{\todocolortext}[3]{\color{2}#3}
% }{
%     % Assert error at todo
%     \newcommand{\todocolortext}[1]{Do NOT use \\#1 for public version!}
% }

% Paper presentation
\ifthenelse{\boolean{PublicVersion}}{
    \setboolean{RevisedVersion}{false}
    \setboolean{CommentVersion}{false}
}{
    \newcommand{\draftversion}{ConfName}

    % For date time print
    % \edef\pdfilemoddate#1{\pdfcreationdate} % not working in xelatex
    \usepackage[useregional]{datetime2}
    \usepackage{background}
    \backgroundsetup{
        color=gray,
        position=current page.west,
        angle=90,
        nodeanchor=west,
        vshift=-5mm,
        hshift=-20mm,
        opacity=1,
        scale=1.75,
        contents=DRAFT [Ver.{\draftversion}] {\DTMnow} {Page \thepage}
    }
}

% Revision
\ifthenelse{\boolean{RevisedVersion}}{
    \usepackage{soul, color}

    % Register customized commands to soul, so that \hl and \st can process
    % these commands without compilation errors
    %
    % https://tex.stackexchange.com/a/139500
    % arg#2 available values:
    %   0 or 1: font switching commands
    %        7: \textsuperscript or similar commands, e.g., \cite, \ref
    %        8: \footnote
    %        9: accents

    % Reference style commands
    \soulregister{\cite}    {7}
    \soulregister{\ref}     {7}
    \soulregister{\autoref} {7}
    \soulregister{\figref}  {7}
    \soulregister{\secref}  {7}
    \soulregister{\tabref}  {7}
    \soulregister{\pageref} {7}

    % Font switching style commands
    \soulregister{\para}    {1}
    \soulregister{\zixuan}  {1}

    % % https://tex.stackexchange.com/questions/282386/make-soul-highlight-span-lines
    % \makeatletter
    % \def\SOUL@hlpreamble{%
    %     \setul{\dp\strutbox}{\dimexpr\ht\strutbox+\dp\strutbox\relax}%
    %     \let\SOUL@stcolor\SOUL@hlcolor
    %     \SOUL@stpreamble
    % }
    % \makeatother

    % Usage:
    % \st{for paragraph with deleting lines}.}
    % \hl{highlight a paragraph with yellow background.}
} {
    % \renewcommand{\st}[1]{}
    % \renewcommand{\hl}[1]{}
    \newcommand{\st}[1]{\PackageError{napaper}{Do NOT use \\st for public version!}}
    \newcommand{\hl}[1]{\PackageError{napaper}{Do NOT use \\hl for public version!}}
}

% Comments
\ifthenelse{\boolean{CommentVersion}}{
    \newcommand{\inlinecomment} [3] {{\color{#1}\sf \footnotesize #2: #3}}
    \newcommand{\ignore}        [1] {{\color{gray} #1}}
    \newcommand{\updatelater}   [1] {{\color{SunsetVII} #1}}
    \newcommand{\overview}      [1] {{\color{SunsetDarkVII} \bfseries #1}}
}{
    \newcommand{\inlinecomment} [3] {}
    \newcommand{\ignore}        [1] {}
    \newcommand{\updatelater}   [1] {}
    % \newcommand{\updatelater}   [1] {\PackageError{napaper}{Do NOT use \\updatelater for public version!}}
    \newcommand{\overview}      [1] {#1}
}

\newcommand{\zixuan}       [1]{\inlinecomment{SunsetIII}  {Zixuan}{#1}}


==> config/style/figure.tex <==
% https://www.overleaf.com/learn/latex/Questions/How_can_I_get_my_table_or_figure_to_stay_where_they_are%2C_instead_of_going_to_the_next_page%3F
% \usepackage[section]{placeins}

\pgfplotsset{compat=1.15}

% Subfigures
\makeatletter
\let\MYcaption\@makecaption
\makeatother
% \usepackage[font=scriptsize]{caption}
\usepackage[font+=smaller,skip=1pt]{subcaption}
\makeatletter
\let\@makecaption\MYcaption
\makeatother

\graphicspath{{figure/}}

\tikzstyle{every picture}+=[font=\sffamily]

% https://tex.stackexchange.com/a/169711
\renewcommand{\floatpagefraction}{.9}

\newcommand{\nafig}[5]{
    % #1 postion
    % #2 subfigure width, e.g., .48\linewidth
    % #3 figure path
    % #4 label
    % #5 caption
    \begin{subfigure}[#1]{#2}
        \centering
        \includegraphics[width=\linewidth]{#3}
        \caption{\label{#4}#5}
    \end{subfigure}
}

% Top align figure and bottom align caption
% https://tex.stackexchange.com/questions/152818/top-aligned-subfigure-with-bottom-aligned-caption
\ExplSyntaxOn
\NewDocumentCommand{\xsubfigure}{ m m }
 {% #1 is a symbolic key, #2 is a list of key-value pairs
  \roly_xsubfigure:nn { #1 } { #2 }
 }
\NewDocumentCommand{\makerow}{ m }
 {% #1 is a list of symbolic keys
  \roly_makerow:n { #1 }
 }

% define the keys
\keys_define:nn { roly/subfigures }
 {
  width .tl_set:N = \l_roly_subfig_width_tl,
  body .tl_set:N = \l_roly_subfig_body_tl,
  caption .tl_set:N = \l_roly_subfig_caption_tl,
 }

% the needed variables
\dim_new:N \l_roly_row_height_dim
\box_new:N \l_roly_body_box

% this is the inner command that stores the properties
\cs_new_protected:Npn \roly_xsubfigure:nn #1 #2
 {
  \prop_if_exist:cTF { l_roly_subfig_#1_prop }
   {
    \prop_clear:c { l_roly_subfig_#1_prop }
   }
   {
    \prop_new:c { l_roly_subfig_#1_prop }
   }
  \keys_set:nn { roly/subfigures } { #2 }
  \prop_put:cnV { l_roly_subfig_#1_prop } { width } \l_roly_subfig_width_tl
  \prop_put:cnV { l_roly_subfig_#1_prop } { body } \l_roly_subfig_body_tl
  \prop_put:cnV { l_roly_subfig_#1_prop } { caption } \l_roly_subfig_caption_tl
 }

% this is the inner command for producing a row
\cs_new_protected:Npn \roly_makerow:n #1
 {
  % get the heights of the objects on a row
  \dim_zero:N \l_roly_row_height_dim
  \clist_map_inline:nn { #1 }
   {
    \hbox_set:Nn \l_roly_body_box
     {
      \prop_item:cn { l_roly_subfig_##1_prop } { body }
     }
    \dim_compare:nT { \box_ht:N \l_roly_body_box > \l_roly_row_height_dim }
     {
      \dim_set:Nn \l_roly_row_height_dim { \box_ht:N \l_roly_body_box }
     }
   }
  % produce a line
  \clist_map_inline:nn { #1 }
   {
    % a subfigure is set here
    \begin{subfigure}[t]{ \prop_item:cn { l_roly_subfig_##1_prop } { width } }
    \raggedright
    \vspace{0pt} % for top alignment
    % the body is set in a suitably dimensioned parbox
    \parbox[t][\l_roly_row_height_dim]{\textwidth}{
      \prop_item:cn { l_roly_subfig_##1_prop } { body }
    }
    % add the caption
    \caption{ \prop_get:cn { l_roly_subfig_##1_prop } { caption } }
    \end{subfigure}
    \hspace{2em} % some space between the objects in a row
   }
   \unskip\\ % end up the row
 }
\ExplSyntaxOff


==> config/style/fonts.tex <==
%%% FONTS
%% https://www.learnui.design/blog/times-new-roman-similar-fonts.html
% \usepackage[T1]{fontenc}
% \usepackage{\RootPath/font/autoinst_output/tex/latex/AdobeCaslonPro/AdobeCaslonPro}
% \usepackage{AdobeCaslonPro}
% \usepackage{merriweather}
% \usepackage{PTSerif}
% \usepackage{LibertinusSerif}
% \usepackage{inconsolata}

% http://www.khirevich.com/latex/microtype/
% \usepackage[kerning,spacing,final]{microtype}
% \usepackage[activate={true,nocompatibility},final,tracking=true,factor=1100,stretch=10,shrink=10]{microtype}
% \usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
% ArXiV by default does not support microtype, need \pdfoutput=1
% https://info.arxiv.org/help/submit_tex.html
\microtypesetup{
    activate={true,nocompatibility},
    final,
    tracking=true,
    kerning=true,
    spacing=true,
    factor=1100,
    stretch=10,
    shrink=10
}
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default is 20/20)

\newcommand*\mycircinternal[1]{%
  \tikz[baseline=(char.base)]{%
  \node[minimum size=0.325cm,shape=circle,draw,inner sep=0.25pt,fill=black,text=white,font=\bfseries] (char) {\small#1};}%
\newcommand*\mycirc[1]{%
\raisebox{.5pt}{\mycircinternal{\raisebox{-.9pt} {#1}}}%
}}

% Check mark and cross mark
% \usepackage{pifont}
% \newcommand{\cmark}{\ding{51}}
% \newcommand{\xmark}{\ding{55}}


==> config/style/space.tex <==
% https://tex.stackexchange.com/a/24468
\setlength{\intextsep}{5pt} % Vertical space above & below [h] floats
% \setlength{\textfloatsep}{5pt} % Vertical space below (above) [t] ([b]) floats
% \setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{5pt}

% % Requires caption package
% \captionsetup{
%     belowskip=0pt
% }

% https://www.overleaf.com/learn/latex/Questions/How_can_I_get_my_table_or_figure_to_stay_where_they_are%2C_instead_of_going_to_the_next_page%3F
% \usepackage[section]{placeins}


==> config/template/acmconf/config.tex <==
\LoadClass[
    sigconf,
    natbib=false,
    nonacm=true,
    % review,
    % anonymous,
]{acmart}

\usepackage[
    backend=biber,
    datamodel=acmdatamodel,
    style=acmnumeric,
]{biblatex}
\bibliography{content/ref.bib}

\acmSubmissionID{\SubmissionID{}}
\renewcommand\footnotetextcopyrightpermission[1]{}

\renewcommand{\napaperbib}{
    % \bibliographystyle{plainurl}
    % \bibliography{content/ref.bib}
    \printbibliography{}
}


==> config/template/asplos/config.tex <==
% ASPLOS Style
\LoadClass[pageno]{config/asplos/template/jpaper}
\newcommand{\asplossubmissionnumber}{XXX}

\usepackage[normalem]{ulem}

% Bib
\newcommand{\napaperbib}{
    \bibliographystyle{plain}
    \bibliography{content/ref.bib}
}
% Page style
\newcommand{\napaperpagestyle}{
    \thispagestyle{empty}
}


==> config/template/cv/config.tex <==
\LoadClass[letterpaper,11pt]{article}

\usepackage{latexsym}
\usepackage[empty]{fullpage}
\usepackage{titlesec}
\usepackage{marvosym}
\usepackage[usenames,dvipsnames]{color}
\usepackage{verbatim}
% \usepackage{enumitem} % Defined by paper.cls
% \usepackage{enumitem-zref} % Deprecated package since 2015
\usepackage[hidelinks]{hyperref}
\usepackage{fancyhdr}
\usepackage{amssymb}
\usepackage{makecell}
\usepackage{xparse}
\usepackage{cleveref}

\renewcommand\familydefault{\sfdefault}
\usepackage[T1]{fontenc}

%% Helvet font, scaled to fit long publication title
\usepackage[scaled=.92]{helvet}

%% Libre Franklin:  https://www.nngroup.com/articles/best-font-for-online-reading/
% \usepackage{librefranklin}

\urlstyle{same}
\newcommand{\rurl}[1]{\href{http://#1}{\nolinkurl{#1}}}

\pagestyle{fancy}
\fancyhf{} % clear all header and footer fields
\fancyfoot{}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}

% Adjust margins
\usepackage[letterpaper,margin=.5in, headsep=.1in]{geometry}
% \addtolength{\oddsidemargin}{-0.6in}
% \addtolength{\evensidemargin}{-0.6in}
% \addtolength{\textwidth}{1.2in}
% \addtolength{\topmargin}{-.6in}
% \addtolength{\textheight}{1.0in}

\raggedbottom
\raggedright
\setlength{\tabcolsep}{0in}

\newlength{\SectionPadding}
\setlength{\SectionPadding}{-1em}

% Sections formatting
\titleformat{\section}{
    \vspace{-6pt}\scshape\raggedright\Large\bfseries
}{}{0em}{}[\color{black}\titlerule \vspace{-5pt}]

\titleformat{\subsection}{
    \vspace{-3pt}\scshape\raggedright\large\itshape
}{}{0em}{}[\vspace{-3pt}]

% Adjust tabular in subheading
% \setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{0.9}

%-------------------------
% Custom commands
\newcommand{\resumeItem}[2]{
    \item\small{
        \textbf{#1}{: #2 \vspace{-2pt}}
    }
}

\newcommand{\resumeItemSimple}[1]{
    \item\small{
        {#1 \vspace{0pt}}
    }
}

\newcommand{\ItemTableWidth}{\textwidth}

\newcommand{\resumeSubheading}[4]{
    \item
    \begin{tabular*}{\ItemTableWidth}{l@{\extracolsep{\fill}}r}
        \textbf{#1} & #2 \\
        \textit{\small#3} & \textit{\small #4} \\
    \end{tabular*}\vspace{-7pt}
}

\newcommand{\resumeSubheadingSimple}[3]{
    \item
    \begin{tabular*}{\ItemTableWidth}{l@{\extracolsep{\fill}}r}
        \textbf{#1} &  \textit{\small #2} \\
        \textit{\bfseries\small#3} & ~ \\
    \end{tabular*}\vspace{-6pt}
}

\newcommand{\resumePublication}[4]{
    \item \label{pub:#1}
    \begin{tabular*}{.8\textwidth}{l@{\extracolsep{\fill}}r}
        \multicolumn{2}{l}{\bfseries \small #2}\\
        {\small \itshape #4} & \textit{#3} \\
    \end{tabular*}\vspace{-7pt}
}

\newcommand{\resumeTalks}[2]{
    \item
    \begin{tabular*}{\ItemTableWidth}{p{\textwidth}@{\extracolsep{\fill}}}
        {\bfseries #1}\\
        \textit{\small#2} \\
    \end{tabular*}\vspace{-7pt}
}

\newcommand{\resumeProject}[3]{
    \item
    \begin{tabular*}{\ItemTableWidth}{l@{\extracolsep{\fill}}r}
        \textbf{#1} &  \textit{\small #2} \\
        \textit{\small#3} & ~ \\
    \end{tabular*}\vspace{-7pt}
}


\newcommand{\resumeSubItem}[2]{\resumeItem{#1}{#2}\vspace{-5pt}}

% \renewcommand{\labelitemi}{}
\renewcommand{\labelitemii}{$\circ$}

\newcommand{\resumeSubHeadingListStart}{\begin{itemize}[leftmargin=0pt,label={},topsep=0pt,itemsep=1pt]}
\newcommand{\resumeSubHeadingListEnd}{\end{itemize}}

\newcommand{\resumeItemListStart}{\begin{itemize}\vspace{0pt}}
\newcommand{\resumeItemListEnd}{\end{itemize}\vspace{0pt}}

\newenvironment{DetailList}
    % {\begin{itemize}[wide, labelindent=\parindent]\vspace{0pt}\small}
    {\begin{itemize}[leftmargin={1em},itemsep=0pt,topsep=2pt,parsep=0pt,partopsep=0pt]\vspace{0pt}\small}
    {\end{itemize}\vspace{0pt}}

\newcommand{\DetailItem}{\resumeItemSimple}

% Content settings
\NewDocumentCommand{\CVNewSection}{mO{#1}}{
    \newenvironment{#1}
    {
        \section{#2}
        \resumeSubHeadingListStart
    }
    {
        \resumeSubHeadingListEnd
        \vspace{\SectionPadding}
    }
}

\NewDocumentCommand{\CVNewSectionTitle}{mO{#1}}{
    \newenvironment{#1}
    {
        \section{#2}
    }
    {
    }
}

\NewDocumentCommand{\CVNewSubSection}{mO{#1}}{
    \newenvironment{#1}
    {
        \subsection{#2}
        \resumeSubHeadingListStart
    }
    {
        \resumeSubHeadingListEnd
        \vspace{\SectionPadding}
    }
}

\CVNewSection{Education}
\newcommand{\EducationItem}{\resumeSubheading}

\CVNewSectionTitle{Interest}
\newcommand{\InterestItem}{\resumeSubheading}

\CVNewSectionTitle{Experience}
\CVNewSubSection{ResearchExperience}[Research Experience]
\CVNewSubSection{IndustrialExperience}[Industry Experience]
\newcommand{\ExperienceItem}{\resumeSubheading}

\CVNewSection{Service}[Services]
\newcommand{\ServiceItem}{\resumeSubheading}

\CVNewSection{Teaching}
\newcommand{\TeachingItem}{\resumeSubheading}

\CVNewSectionTitle{Publication}[Publications]
\newenvironment{PublicationList}[1]
{
    \begin{enumerate}[leftmargin=3em,label={\small[#1\arabic*]},topsep=0pt,itemsep=1pt,topsep=2pt,parsep=0pt,partopsep=0pt]
}
{
    \end{enumerate}
    \vspace{\SectionPadding}
}
\newcommand{\PublicationItem}[4]{
    \item \small \label{pub:#1} {#4}. {#2}, \textit{#3}
}
\newcommand{\PublicationItemOngoing}[4]{
    \item \small \label{pub:#1} {#4}. {#2}
}

\CVNewSection{Mentorship}[Mentorships]
\newcommand{\MentorshipItem}{\resumeSubheading}

\CVNewSection{Talk}[Invited Talks]
\newcommand{\TalkItem}{\resumeTalks}

\CVNewSection{Honor}[Honors]
\newcommand{\HonorItem}{}

\newenvironment{SectionTable}
    {\begin{tabular*}{\ItemTableWidth}{l@{\extracolsep{4em}}l}}
    {\end{tabular*}}
\newenvironment{Reference}
    {\section{References}\begin{SectionTable}}
    {\end{SectionTable}}
\newcommand{\ReferenceItem}[2]{\textbf{#1} & #2 \\}


==> config/template/eurosys/config.tex <==
\LoadClass[sigplan,review,anonymous]{acmart}
\acmSubmissionID{XXX}
\renewcommand\footnotetextcopyrightpermission[1]{}


==> config/template/ieee/config.tex <==
% IEEE conference -- MICRO2020 camera ready
\LoadClass[conference]{config/ieee/template/IEEEtran}
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% Bib
\newcommand{\napaperbib}{
    \bibliographystyle{IEEEtranS}
    \bibliography{content/ref.bib}
}
% Page style
\newcommand{\napaperpagestyle}{
    % None specified
}


==> config/template/ieee/template/bib/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> config/template/isca/config.tex <==
% ISCA Style
\LoadClass[conference]{config/isca/template/IEEEtran}

% From ISCA 2020 Template
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{fancyhdr}
\usepackage[hyphens]{url}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% Ensure letter paper
\pdfpagewidth=8.5in
\pdfpageheight=11in


%%%%%%%%%%%---SETME-----%%%%%%%%%%%%%
\newcommand{\iscasubmissionnumber}{XXX}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\fancypagestyle{firstpage}{
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\fancyhead[C]{\normalsize{ISCA 2020 Submission
    \textbf{\#\iscasubmissionnumber} \\ Confidential Draft: DO NOT DISTRIBUTE}}
\fancyfoot[C]{\thepage}
}

\pagenumbering{arabic}
% Bib
\newcommand{\napaperbib}{
    \bibliographystyle{IEEEtranS}
    \bibliography{content/ref.bib}
}
% Page style
\newcommand{\napaperpagestyle}{
    \thispagestyle{firstpage}
    \pagestyle{plain}
}


==> config/template/letter/config.tex <==
% https://www.matthewjmiller.net/howtos/customized-cover-letter-scripts/
\LoadClass[10pt,stdletter,orderfromtodate,sigleft]{newlfm}
\usepackage{kpfonts}
\usepackage{url}

\newlfmP{MinFoot=0pt}
\newlfmP{footermarginsize=15pt}
\newlfmP{unprbottom=0pt}
% \usepackage{layout}
% \usepackage{showframe}

\widowpenalty=1000
\clubpenalty=1000

\newlfmP{headermarginskip=0pt}
\newlfmP{topmarginskip=0pt}
\newlfmP{bottommarginskip=0pt}

\newlfmP{addrfromskipbefore=0pt}
\newlfmP{addrfromskipafter=0pt}
\newlfmP{addrtoskipbefore=5pt}
\newlfmP{addrtoskipafter=10pt}
\newlfmP{dateskipbefore=10pt}
\newlfmP{dateskipafter=5pt}

\newlfmP{sigsize=0pt}
\newlfmP{sigskipbefore=0pt}
\newlfmP{sigskipafter=0pt}
\newlfmP{postsigskipbefore=0pt}
\newlfmP{postsigskipafter=0pt}
\newlfmP{closeskipbefore=5pt}
\newlfmP{closeskipafter=0pt}

% \newlfmP{greettoskipafter=0pt}

\newlfmP{addrfromphone}
\newlfmP{addrfromemail}
\PhrPhone{Phone}
\PhrEmail{Email}

\namefrom{Zixuan Wang}
\addrfrom{%
    Department of Computer Science and Engineering\\
    University of California, San Diego\\
    9500 Gilman Drive\\
    La Jolla, CA 92122
}
\phonefrom{725-600-1695}
\emailfrom{zxwang@ucsd.edu}

\greetto{Dear Members of the Search Committee,}
\closeline{Sincerely,}
% \signame{Zixuan Wang\vspace{-20pt}}

% #1: TargetDepartment
% #2: TargetUniversity
% #3: TargetAddress
\newcommand{\TargetAddress}[3]
{
\newcommand{\TargetDepartment}{#1}
\newcommand{\TargetUniversity}{#2}
\newcommand{\TargetMailAddress}{#3}
\addrto{%
Faculty Search Committee\\
\TargetDepartment\\
\TargetUniversity\\
\TargetMailAddress}
}

% \usepackage{epstopdf}
% \epstopdfsetup{update}
\usepackage{graphicx}

\newsavebox{\LetterLOGO}
\sbox{\LetterLOGO}{%
    \parbox[b]{1.75in}{%
        \vspace{0.5in}%
        \includegraphics[scale=.5]{\RootPath/figure/fig/ucsd/UCSanDiegoLogo-Black.pdf}%
    }%
}%
\makeletterhead{UCSDLOGO}{\Lheader{\usebox{\LetterLOGO}}}
\lthUCSDLOGO


==> config/template/micro/config.tex <==
% % Micro 2020 Style
\LoadClass{config/micro/template/sig-alternate}
\usepackage{mathptmx} % This is Times font

\usepackage{fancyhdr}
\usepackage[normalem]{ulem}
\usepackage[hyphens]{url}
\usepackage[sort,nocompress]{cite}
\usepackage[final]{microtype}
\usepackage[keeplastbox]{flushend}
% Always include hyperref last
\usepackage[bookmarks=true,breaklinks=true,letterpaper=true,colorlinks,linkcolor=black,citecolor=blue,urlcolor=black]{hyperref}

% Ensure letter paper
\pdfpagewidth=8.5in
\pdfpageheight=11in

%%%%%%%%%%%---SETME-----%%%%%%%%%%%%%
\newcommand{\microsubmissionnumber}{XXX}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\fancypagestyle{firstpage}{
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \fancyhead[C]{\vspace{15pt}\normalsize{MICRO 2020 Submission
        \textbf{\#\microsubmissionnumber} -- Confidential Draft -- Do NOT Distribute!!}}
    \fancyfoot[C]{\thepage}
}

\pagenumbering{arabic}

% Bib
\newcommand{\napaperbib}{
    \bibliographystyle{IEEEtranS}
    \bibliography{content/ref.bib}
}
% Page style
\newcommand{\napaperpagestyle}{
    \thispagestyle{firstpage}
    \pagestyle{plain}
}


==> config/template/sp/config.tex <==
% IEEE S&P
\LoadClass[conference]{config/ieee/template/IEEEtran}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage[table]{xcolor}
% Bib
\newcommand{\napaperbib}{
    \bibliographystyle{IEEEtranS}
    \bibliography{content/ref.bib}
}
% Page style
\newcommand{\napaperpagestyle}{
    \thispagestyle{firstpage}
    \pagestyle{plain}
}


==> config/template/statement/config.tex <==
\LoadClass[letterpaper,10pt]{article}
\usepackage[letterpaper,margin=.85in, headsep=.1in]{geometry}
\usepackage{xcolor}
\usepackage{fancyhdr}
\usepackage[sorting=none, backend=biber, style=numeric-comp, maxbibnames=99]{biblatex}

% Bib
\usepackage{etoolbox}
\patchcmd{\thebibliography}
  {\settowidth}
  {\setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}\settowidth}
  {}{}
\apptocmd{\thebibliography}
  {\small}
  {}{}
\addbibresource{\RootPath/content/ref.bib}
\newcommand{\napaperbib}{
    \clearpage
    % \renewcommand{\emph}[1]{\textit{#1}}
    \printbibliography[heading=bibliography]
}

% \newcommand{\soptitle}{Research Statement}
\newcommand{\yourname}{Zixuan Wang}
\newcommand{\youremail}{zxwang@ucsd.edu}
\newcommand{\yourweb}{https://www.thenetadmin.com}

\newcommand{\statement}[1]{\par\medskip
  \underline{\textcolor{blue}{\textbf{\#1:}}}\space
}

% \renewcommand{\maketitle}{
%     \begin{center}
%         {\LARGE \@title}\\
%         {\smallskip}
%         {\large \@author}
%     \end{center}
%     \hrule
%     \vspace{1pt}
%     \hrule height 1pt
%     \bigskip
% }

\definecolor{color1}{RGB}{0,0,90} % Color of the article title and sections
\definecolor{color2}{RGB}{0,20,20} % Color of the boxes behind the abstract and headings

\renewcommand{\maketitle}{%
    \thispagestyle{empty}%
    \vskip-48pt%
    % {\raggedright\color{color1}\sffamily\bfseries\fontsize{20}{25}\selectfont \@title\par}%
    {\raggedright\color{color1}\sffamily\bfseries\LARGE\selectfont \@title\par}%
    \vskip5pt%
    {\raggedright\color{color1}\sffamily\fontsize{12}{16}\selectfont \@author\par}%
    \vskip5pt%
}

\usepackage[
  colorlinks,
  breaklinks,
  urlcolor=black,
  linkcolor=black,
  citecolor=black,
  % pdftitle={\yourname - \soptitle},
  pdfauthor={\yourname},
  unicode
]{hyperref}

% Fonts
\usepackage{fontspec}
\defaultfontfeatures{Mapping=tex-text,Scale=MatchLowercase}
\setmainfont[Path=\RootPath/font/, BoldFont={*-Bold}, ItalicFont={*-Italic}, BoldItalicFont={*-BoldItalic}]{ACaslonPro}
% \renewcommand\familydefault{\sfdefault}
\usepackage{helvet}
% \usepackage{tgschola} % or any other font package you like

% Page Style
\newcommand{\napaperpagestyle}{
    \thispagestyle{empty}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt} % No header rule
    \renewcommand{\footrulewidth}{0pt} % No footer rule
    \fancyhead[C]{%
    %   \footnotesize\sffamily
    %   \@author%
    %   \hfill%
    %   \@title%
    %   \hfill%
    %   \yourweb%
    }
    \rhead{\small\sffamily\bfseries\@title\ --- \@author}
}

% Disable indentation
\usepackage{parskip}


% \newcommand{\theme}[1]{{\vspace{5pt}\noindent \large \textbf{#1}}}
% \newcommand{\research}[1]{{\vspace{5pt}\noindent \Large \textbf{#1}}}
% \newcommand{\para}[1]{\vspace{3pt}\noindent\textbf{#1}}
% \newcommand{\para}[1]{\vspace{3pt}\noindent\textbf{{{{#1}}\hspace{0.5em}}}}
% \newcommand{\subpara}[1]{\vspace{3pt}\noindent\textit{#1}}

\usepackage[explicit]{titlesec}
\titleformat{\section}
    {\color{color1}\large\sffamily\bfseries}
    {}
    {0em}
    {#1}
    []

\titleformat{\subsection}
    {\color{color1}\sffamily\bfseries}
    {}
    {0em}
    {#1}
    []

\newcommand{\research}[1]{{\vspace{3pt}\noindent\color{color1}\sffamily\bfseries\Large #1}}
\newcommand{\theme}[1]{{\vspace{3pt}\noindent\sffamily\bfseries\large #1}}
\newcommand{\para}[1]{{\noindent\sffamily\small\bfseries #1}}


==> config/template/usenix/config.tex <==
% USENIX conference, e.g. ATC
\LoadClass[letterpaper,twocolumn,10pt]{article}
\usepackage{config/usenix/template/usenix-2020-09}
% Bib
\renewcommand{\napaperbib}{
    \bibliographystyle{plainurl}
    \bibliography{content/ref.bib}
}
% Page style
\renewcommand{\napaperpagestyle}{
    \thispagestyle{empty} % Camera ready style
    \pagestyle{empty}     % Camera ready style
}


==> content/1-intro-comment.tex <==

\updatelater{
% My ongoing research is leveraging CXL to develop architecture and system support to simplify heterogeneous programming.
% My ongoing research is rethinking the programming interface to abstract architecture details and simplify the heterogeneous programming.
My ongoing research focuses on simplifying programming for heterogeneous systems by rethinking the programming interface to abstract architectural details.
%
\zixuan{One sentence TL;DR; of the impact.}
%
I have observed that programming multi-accelerator systems is akin to multi-threading programming of multi-CPU systems.
%
% Multi-threading allows threads to be declared as a small piece of code focusing on a specific aspect of the application's functionality, and relies on CPU cache-coherence to provide the thread full access to the shared code and system resource.
Multi-threading allows threads to handle specific aspects of an application's functionality and relies on CPU cache-coherence to access shared code and system resources.
%
% The multi-threading programming model provides an abstraction of distributing tasks: each thread's workload is defined by a small piece of code, while at runtime, threads are distributed to different CPU cores, can access the entire process memory and system resources.
%
% The key architecture that enables such multi-threading programming is the cache-coherent interconnection across CPU cores.
% Cache-coherent interconnection across CPU cores is the key architecture that enables the multi-threading.
%
% Now CXL enables a broader cache-coherent interconnection across different accelerator architectures, including CPUs, I see a chance of programming heterogeneous systems using a multi-threading programming model:
With CXL enabling cache-coherent interconnection across diverse accelerator architectures, including CPUs, a multi-threading programming model for heterogeneous systems seems feasible.
%
% each accelerator runs a thread of the application and communicates with other threads through standard multi-threading techniques such as shared memory and locks.
In this model, each accelerator runs an application thread, communicating with others using standard multi-threading techniques like shared memory and locks.
%
% The accelerator thread is defined by a small piece of code, similar to defining a CPU thread task, while able to leverage system functionalities such as filesystems without custom code.
The code for each accelerator thread is defined similarly to a CPU thread task, with transparent access to system functionalities like filesystems without custom code.
% This model allows an accelerator thread to not only utilize the accelerator functionalities, but also access system resources such as filesystems without needing custom solutions.
% It also enables easy interaction with threads on different devices, all while leveraging the well-established multi-threading concept.
% This allows the programmer to implement the accelerator job as a thread, which requires
%
To implement this, I plan to develop a software-based language runtime system based on WebAssembly~\cite{wasi} that allocates application threads across different CXL-connected accelerators.
% runtime system
% that leverages CXL to coordinate different types of accelerators while preserving a unified programming interface to the application.
%
This further enables conventional multi-threading programs, originally written for multi-CPU systems, to use the multi-accelerator heterogeneous system without modifications.


Taking this concept further, my goal is to develop a \emphu{scalable system} for future heterogeneous computing where new accelerators can be integrated without application code modifications or recompilations.
%
% The hardware-level support of such a system is commercially available based on the emerging cache-coherent interconnections such as CXL, and my prior research work~\cite{COARSE} proved such interconnections significantly improve the performance of machine learning systems.
%
% But the system- and programming-level supports are yet to be explored toward a more generic system.
%
% \zixuan{``This research fills the gap ... Long needed by ...''}
% This research opens a new practice of heterogeneous computing by shifting the complexity of utilizing new accelerators from the application to the language runtime system, thus allowing applications to leverage diverse accelerators without modifying code.
This approach shifts the complexity of using new accelerators from the application to the language runtime system, allowing applications to harness diverse accelerators without code changes.
%
The runtime system further scales the application performance by sending the code to where the data is, such as scheduling file access threads to accelerators in storage devices and assigning networking threads to processors in network cards.
%
% This model incentivizes application developers to explore their code in heterogeneous systems without the need to learn accelerators' specialized programming models.
It encourages application developers to explore heterogeneous systems without learning specialized programming models for each accelerator.
%
% On the other hand, this model allows accelerator developers to easily identify the performance bottleneck in application code and build new accelerators without worrying about the usability of software applications.
Additionally, it enables accelerator developers to focus on identifying performance bottlenecks in application code and designing new accelerators without software usability concerns.
%
% In the long term, this model achieves much more diverse accelerators in the system with minimal programming effort from applications and minimal integration effort from accelerators, thus scaling the computing performance to a level that current heterogeneous computing cannot achieve.
%
% In the long term, this research opens new research opportunities, such as profiling-guided thread scheduling, just-in-time compilation for accelerators, abstracting common operations in accelerators, and more.
This research paves the way for innovative opportunities, including performance-guided thread scheduling, just-in-time compilation for accelerators, abstracting common operations in accelerators, and more.
%
% This research allows applications to leverage accelerators without the need to know their existence
% This research further scales the application performance by sending the code to where the data is--scheduling file access threads to accelerators in storage devices and assigning networking threads to processors in network cards--all without implementing specialized code for specific accelerator architectures.

% \zixuan{``Code is future-proof''}

% \zixuan{``We have devoted xxx efforts on building such a system. Preliminary results show that...''}

% \zixuan{``The future direction.''}

% \zixuan{Claim benefit of WebAssembly: https://www.secondstate.io/articles/fast-llm-inference/}
}


==> content/4-implementation.tex <==
\section{Implementation}

==> content/6-related.tex <==
\section{Related Work}

==> content/figure/evaluation.tex <==
% \newcommand{\evalConfig}{
%     \ctable[
%         % caption = {System for Evaluation},
%         % label = {tab:system-configuration},
%         width = \linewidth{},
%         doinside = \scriptsize,
%         pos = t
%     ]{lX<{\centering}}{
%         % No table footnote
%     }{
%                                                                                 \FL
%         \multirow{2}{*}{CPU}            & Intel SapphireRapids 4416+             \NN
%         % ~                               & 950 KiB L1D\$, 40 MiB L2\$, 37.5 L3\$  \NN
%         ~                               & 2 Sockets, 20 cores per socket         \ML
%         Memory                          & 256 GiB DDR5                           \ML
%         \multirow{3}{*}{CXL}            & Intel Agilex-7 FPGA                    \NN
%         ~                               & CXL hard IP type 2 \& type 3           \NN
%         ~                               & 64 GiB DDR4 SODIMM                     \ML
%         OS                              & Ubuntu 22.04, Linux 6.7                \LL
%     }
% }

% \newcommand{\evalCXLPerf} {
%     \ctable[
%         % caption = {CXL Performance},
%         % label = {tab:system-configuration},
%         width = \linewidth{},
%         doinside = \scriptsize,
%         pos = t
%     ]{lX<{\centering}X<{\centering}}{
%         % No table footnote
%     }{
%                                                     \FL
%         ~           & \multicolumn{2}{c}{Performance}  \tabularnewline \cmidrule{2-3}
%         Component   & Latency (ns) & Bandwidth (GiB/s) \ML
%         Local DDR5  &        108.2 &             105.0 \NN
%         Remote DDR5 &        171.5 &              59.1 \NN
%         Local CXL   &        371.2 &              17.4 \NN
%         Remote CXL  &        538.0 &               9.0 \LL
%     }
% }

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{.24\linewidth}
        \centering
        \resizebox{\textwidth}{!}{
            \scriptsize
            \begin{tabular}{|l|c|}
                                                                                        \hline
                \multirow{2}{*}{CPU}            & Intel SapphireRapids 4416+             \\
                % ~                               & 950 KiB L1D\$, 40 MiB L2\$, 37.5 L3\$  \\
                ~                               & 2 Sockets, 20 cores per socket         \\\hline
                Memory                          & 256 GiB DDR5                           \\\hline
                \multirow{3}{*}{CXL}            & Intel Agilex-7 FPGA                    \\
                ~                               & CXL hard IP type 2 \& type 3           \\
                ~                               & 64 GiB DDR4 SODIMM                     \\\hline
                OS                              & Ubuntu 22.04, Linux 6.7                \\\hline
            \end{tabular}
        }
        \vspace{4pt}
        \caption{System configuration.}
        \label{subfig:system-configuration}
    \end{subfigure}
    \hfill
    \begin{subtable}[b]{.24\linewidth}
        \centering
        \resizebox{\textwidth}{!}{
            \scriptsize
            \begin{tabular}{|l|cc|}
                                \hline
                ~           & \multicolumn{2}{c|}{Performance}  \\ \cline{2-3}
                Component   & Latency (ns) &        BW (GiB/s) \\ \hline
                Local DDR5  &        108.2 &             105.0 \\
                Remote DDR5 &        171.5 &              59.1 \\
                Local CXL   &        371.2 &              17.4 \\
                Remote CXL  &        538.0 &               9.0 \\ \hline
            \end{tabular}
        }
        \vspace{16pt}
        \caption{CXL Performance.}
        \label{subfig:cxl-perf}
    \end{subtable}
    \hfill
    \begin{subfigure}[b]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/plot/wasi-llc-miss.tikz.pdf}
        \caption{CPU LLC miss ratio.}
        \label{subfig:wasi-llc-miss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/plot/wasi-ptr-chasing.tikz.pdf}
        \caption{Memory access latency.}
        \label{subfig:wasi-ptr-chasing}
    \end{subfigure}

    \caption{WASI performance as a runtime system.}
    \label{fig:wasi-perf}
\end{figure*}


==> content/figure/system-overview.tex <==
\begin{figure*}[t]
    \centering
    \nafig{b}{.24\linewidth}{example-image-a}{subfig:codeflow-system}{CodeFlow system stack.}
    \nafig{b}{.24\linewidth}{example-image-a}{subfig:conventional-code}{Conventional code Example.}
    \nafig{b}{.24\linewidth}{example-image-a}{subfig:codeflow-code}{CodeFlow code Example.}
    \nafig{b}{.24\linewidth}{example-image-a}{subfig:codeflow-schedule}{CodeFlow scheduling.}
    \caption{CodeFlow overview.}
    \label{fig:system overview}
\end{figure*}


==> content/table/compare-hetero-cpu.tex <==
\ctable[
    caption = {Heterogeneous Computing vs Multi-Threading},
    label = {tab:compare-hetero-cpu},
    width = \linewidth{},
    pos = ht
]{llc}{
    % No table footnote
    \zixuan{Maybe not a good table for intro, move to motivation?}
}{
                                                                            \FL
    Component                       & Observation         & LENS vs. NVLeak \ML
    WPQ                             & Size                & Reproduced      \ML
    ~                               & Timing Sensitive    & New             \LL
}

% Line endings \FL \ML \LL, and empty line \NN

==> figure/fig/Makefile <==

.DEFAULT_GOALS:=all

pdfs := # All pdfs under 'lucidchart' folder

flatten_pdfs := codeflow-overview.flatten.pdf \
                codeflow-system-stack.flatten.pdf \
		hetero-system-stack.flatten.pdf

curr_dir := $(shell dirname $(realpath $(firstword $(MAKEFILE_LIST))))
gs_script := $(realpath $(curr_dir)/../../script/figure/ghostscript/embed_font.sh)

.PHONY: all
all: $(pdfs) $(flatten_pdfs)

%.pdf: lucidchart/%.pdf
	bash $(gs_script) "$<" "$@"

%.flatten.pdf: %.pdf
	pdf2ps $< - | ps2pdf - $@


==> figure/fig/tex/Makefile <==

pdfs := \
	hetero-code-example.pdf \
	multi-thread-code-example-cpp.pdf

.PHONY: all
all: $(pdfs)

%.pdf: src/%.tex
	@ echo GEN $@
	pushd src && \
	latexmk --quiet --shell-escape -pdf $$(basename $<) && \
	mv $@ $@.pre.pdf && \
	bash ../../../../script/figure/ghostscript/embed_font.sh $@.pre.pdf $@ && \
	popd
	mv src/$@ .

